Synchronization-Aware and Algorithm-Efficient Chance Constrained Optimal Power Flow

One of the most common control decisions faced by power system operators is the question of how to dispatch generation to meet demand for power. This is a complex optimization problem that includes many nonlinear, non convex constraints as well as inherent uncertainties about future demand for power and available generation. In this paper we develop convex formulations to appropriately model crucial classes of nonlinearities and stochastic effects. We focus on solving a nonlinear optimal power flow (OPF) problem that includes loss of synchrony constraints and models wind-farm caused fluctuations. In particular, we develop (a) a convex formulation of the deterministic phase-difference nonlinear Optimum Power Flow (OPF) problem; and (b) a probabilistic chance constrained OPF for angular stability, thermal overloads and generation limits that is computationally tractable.

==> 05Robust.tex <==

\section{V. Robustification of the OPF and CC-OPF}

{\color{red}  ... do we have this Section or not?  Dan - this is your call.}

\subsection{Robust (Convex and Tractable !) AC-OPF}

%{\color{red} ... may have it ... or may drop it ... leave this part for Dan to fill in /add/decide ... robustness discussed in here will be with respect to the wind ... I suppose ...}

\subsection{Robust CC-OPF}

%{\color{red}  ... here we simply reiterate some of the arguments from \cite{12BCH} ... with direct reference ... and reserving the whole Section for that is,  probably, not worth it}

